Learning-Based Robust Fixed-Time Terminal Sliding Mode Control

In this paper, we develop and analyze an integral fixed-time sliding mode control method for a scenario in which the system model is only partially known, utilizing Gaussian processes. We present two theorems on fixed-time convergence. The first theorem addresses the fully known system model, while the second considers situations where the system's drift is approximated utilizing Gaussian processes (GP) for approximating unknown dynamics. Both theorems establish the global fixed-time stability of the closed-loop system. The stability analysis is based on a straightforward quadratic Lyapunov function. Our proposed method outperforms an established adaptive fixed-time sliding mode control approach, especially when ample training data is available.

==> Notation.tex <==
{\textcolor{black}{ 
\subsection*{Notations}
Let $\mathbb{R}$ denote the set of real numbers, and define $\mathbb{R}_{+}$ as the set of non-negative real numbers, i.e., $\mathbb{R}_{+}=\{s\in\mathbb{R}:s\geq0\}$, and $\mathbb{R}_{>0}$ as the set of strictly positive real numbers, i.e., $\mathbb{R}_{>0}=\mathbb{R}_+\setminus\{0\}$.
Throughout the paper, the notation $\left\lfloor x\right\rceil^{\alpha} = |x|^{\alpha}\sign(x)$ is utilized, where $\left\lfloor x\right\rceil^{0} = \sign(x)$. The function $\sign(x)$ is defined as follows \cite{shtessel2014sliding}:
\(\sign(x):=-1 \quad  \text{if } \quad x < 0,
\sign(0) \in [-1, 1], \quad
1  \text{if } \quad x > 0\).
}

==> SecII.tex <==
\section{Preliminaries}\label{Sec:II}
\subsection{Fixed- and finite-time stability}
{\textcolor{black}{To review some findings regarding fixed- and finite-time stability, Consider the following system:}
\begin{equation}
\label{eq:fz}
\begin{aligned}
\dot{x}(t) = f(x(t)), \quad x(t) \in \mathbb{R}^n, \quad x(0) = x_0.
\end{aligned}
\end{equation}
with the continuous function $f$.
\begin{definition}
From \cite{bhat2000finite}: {\textcolor{black}{a}} system denoted as \eqref{eq:fz} is considered globally finite-time stable if it satisfies Lyapunov stability and for any initial condition vector $x_0$ in $\mathbb{R}^n$, there exists a settling time function $T(x_0) \geq 0$ dependent on the initial conditions. Specifically, for any solution $x(\cdot)$ of system \eqref{eq:fz} with the initial condition $x(0) = x_0$, it holds that as $t$ approaches $T(x_0)$, the norm of $x(t)$ converges to zero, i.e., $\lim_{t \to T(x_0)} |x(t)| = 0$. In other words, the norm of $x(t)$ remains identically zero for all $t \geq T(x_0)$. The function $T(x_0)$ is referred to as the settling time.
\end{definition}
\begin{definition} {\textcolor{black}{(see \cite{polyakov2011nonlinear}): System \eqref{eq:fz} is considered globally FxT stable if it satisfies the following conditions: 
1) It is globally finite-time stable; 2) The settling-time function \(T(x_0)\) is upper-bounded by a constant \(T_{\max} > 0\), meaning that for all \(x_0 \in \mathbb{R}^n\), \(T(x_0) \leq T_{\max}\), and \(T_{\max}\) remains constant regardless of the initial conditions.
}}
\end{definition}
The following lemmas are necessary for the subsequent analysis.
\begin{lemma}\label{lemma:1} (see \cite{polyakov2011nonlinear}): If there exists a continuously differentiable positive definite radially unbounded function $V: \mathbb{R}^n \to \mathbb{R}^+$ such that
\begin{small}
\[
\dot{V}(x) \leq -c_1V(x)^{h_{\textcolor{black}1}} - c_2V(x)^{h_2} 
\]\end{small}
where $V$ is called the Lyapuov function and $x \in \mathbb{R}^n$, $c_i> 0$, and $0 < h_1 < 1 < h_2$, then system \eqref{eq:fz} is globally FxT stable  {\textcolor{black}{with a settling time bounded by}}
\begin{small}
\begin{align}
T(x_0) \leq \frac{1} {c_1(1 - h_1)} + \frac{1} {c_2(h_2 - 1)}.
\end{align}\end{small}
\end{lemma}
\begin{lemma}\label{lemma:2}\cite{labbadi2023design}
Consider the following system:
\begin{equation}
\dot{x}(t)=-\alpha\frac{\sqrt{\pi}}{2}\exp(x^2)\sign(x)+d(t),\quad x(0)=x_0,\label{eq:sysP}
\end{equation}
where \(\alpha>\tfrac{2}{\sqrt{\pi}}\bar{d}\),   $x\in\R$, and  $d\in\R$.
Then,  system \eqref{eq:sysP} is globally fixed-time stable with a settling time $T(x_0)\leq T_{\max}$ where
\(T_{\max}=\frac{1}{\alpha-\tfrac{2}{\sqrt{\pi}}\bar{d}}.
\)
\end{lemma}
\subsection{Problem statement}
Consider the following perturbed system \cite{khanzadeh2023fixed}.
\begin{equation}
\begin{cases}
\dot{x}_{\textcolor{black}{1}}(t) = f_1(x) + g_1(x)u_1(t) + d_1(t) \\
\dot{x}_{\textcolor{black}{2}} (t) = f_2(x) + g_2(x)u_2(t) + d_2(t) \\
\vdots \\
\dot{x}_n(t) = f_n(x) + g_n(x)u_n(t) + d_n(t)
\end{cases}
\label{eq:model}
\end{equation}
where: 
{\textcolor{black}{$x = [x_1 \ x_2 \ \cdots \ x_n]^T \in \mathbb{R}^n$ is the state,
$u = [u_1 \ u_2 \ \cdots \ u_n]^T \in \mathbb{R}^n$ is the input,
$f_i$ and $g_i$ are known nonlinear functions such that $g_i\neq 0$ for all $x \in \mathbb{R}^n$.
$d_i \in \mathbb{R}^n$ is a perturbation assumed to be bounded but with an unknown upper bound, satisfying $|d_i(t)| \leq \bar{d}_i$ with $(i = \{1, \ldots, n\})$.}} The mathematical model represented by equation \eqref{eq:model} holds significance across various crucial engineering applications, including but not limited to multi-agent systems \cite{defoort2015leader}, synchronization of complex dynamical networks \cite{yang2017fixed}, recurrent neural networks \cite{yang2017fixed}, and beyond. 
This form is commonly found in many practical systems such as robot manipulators, autonomous vehicles, and quadrotors. These systems often exhibit complex dynamics and uncertainties that must be managed effectively to ensure safe and reliable operation. To ensure the applicability of our approach, we make the following assumption regarding the matrix \( g \).

% To design a control law that ensures fixed-time tracking, an adequate model of the uncertainty \( f_i(x)\) is essential. In many real-world applications, it is impractical to derive an exact model of the system's uncertainties due to the complexity and variability of the environment. Therefore, we employ a data-driven model to infer this uncertainty. The model utilizes noisy measurement data \( N \) specified by the following assumption:

% \begin{ass}\label{assum:2} The measurement data \( F \) consists of \( N \in \mathbb{N} \) training pairs \(\{x(k), y(k)\}\) with \( y(k) = f_i(x(k)) + \epsilon(k) \) for \( k = 1, \ldots, N \), where \( \epsilon(k) \) is i.i.d. zero-mean Gaussian noise with covariance \( \Sigma_o = \text{diag}(\sigma^2_{o,1}, \ldots, \sigma^2_{o,m}) \), \( \sigma_{o,j} \in \mathbb{R}^+ \) for \( j = 1, \ldots, m \).
% \end{ass}
% Assumption \ref{assum:2} is a mild assumption often encountered in learning-based control settings \cite{seeger2004gaussian,srinivas2012information}. It allows for Gaussian-distributed measurement noise, which can result from various sources such as numerical differentiation, sensor inaccuracies, or external disturbances. The assumption of Gaussian noise is beneficial because it simplifies the mathematical treatment and enables the use of well-established statistical techniques for uncertainty quantification.

% In some contexts, the requirements for the measurement noise distribution can be relaxed, for instance, by restricting it to be bounded \cite{seeger2004gaussian,srinivas2012information}, but this extension is beyond the scope of this paper. Even with this simplification, the Gaussian noise assumption provides a realistic and manageable way to handle measurement inaccuracies and ensures that the learning-based approach can effectively capture the underlying system uncertainties.

% This approach is particularly beneficial for systems where precise modeling is challenging, and real-time adaptation to changing conditions is required. For example, in smart grid, the ability to adapt to varying road conditions, and sensor noise is critical for fixed-time tracking. 



==> name.tex <==
\begin{equation}\label{eq:V2}
    \begin{aligned}
            \color{red}{i_{fq\text{-r}}} &= \color{red}{C_f \left(\frac{1}{C_f}i_{oq}+\omega_f{x_1}- \gamma_{21} |\er_2(t)|^{\frac{\alpha_{21}\er_2^2(t)}{1+\beta_{21}\er_2^2(t)}} \times\right.}\\ 
    & \quad \left. \left\lfloor \er_2(t)\right\rceil^{\frac{p_2}{q_2}} +\dot{x}_{\text{2-r}}- \gamma_{22} |s_2(\er)|^{\frac{\alpha_{22}s_2^2(\er)}{1+\beta_{22}s_2^2(\er)}}  \left\lfloor s_2(\er)\right\rceil^{0}\right)
    \end{aligned}
\end{equation}
